On the notion of a patterning property in model theory

Different kinds of definable patterns in the models of a first-order theory, such as the order property, the tree property, or the ($n$-)strict order property, allow us to distinguish theories according to their logical complexity. The complexity distinctions given by these definable patterns play a central role in model theory. However, a rigorous definition of the notion of a model-theoretic patterning property has yet to be established. We start by discussing different proposals from the literature for making the notion of a model-theoretic patterning property rigorous. Some examples will include the straight definability of Shelah, which will describe properties definable by a pattern of consistency and inconsistency in a formula and its negation, and the poset definability of Garcia and Mennuni, covering properties definable by interpreting a partial order embedding a given poset. We will also introduce a higher-arity version of straight definability. In our first main result, we will answer open questions of Bailetti and Garcia-Mennuni, showing that the $n$-strict order property $\mathrm{SOP}_{n}$ is straightly definable and poset definable even for integers $n \geq 4$. This will complete the categorization of all of the classical classification-theoretic properties as straightly definable. Our other main result will concern properties that are straightly definable without negation: the positively straightly definable properties defined by Bailetti. We will show using Saracino's theorem and results of Bodirsky, Bodor and Marimon that, in any countably categorical theory, implications between positively straightly definable properties must be exhibited at the level of $\exists\forall$-formulas. This will have special consequences under the assumption that $\mathrm{SOP}_{2}$ is equal to $\mathrm{SOP}_{3}$.

==> deleted_text.tex <==
From trace definition section:


[discuss why TP can't be captured by either. Note that $IP_k$ is characterizable by collapse]

Several well-known classificatory properties, most notably stability and NIP, can be characterized by a \textit{collapse of indiscernibles}, i.e., by the property that, whenever a particular kind of indiscernible structure appears in a model, that indiscernible structure in fact possesses some stronger form of indiscernibility.

Stable theories are characterized by the collapse of indiscernible sequences to indiscernible sets (cf. Shelah), and NIP theories are characterized by the collapse of ordered random graph indiscernibles to indiscernible sequences (cf. Scow).

In these cases, the structures which are being ``collapsed" seem to appear in another kind of characterization of stable and NIP theories, using the notion of \textit{trace definability}, due to \cite{walsberg_notes_2021}.

\begin{definition}
    Let $\calM$ and $\calN$ be $L$ and $L'$ structures, respectively. Let $\tau\colon \calN\to\calM^k$ be an injection. Then $\calM$ \textbf{trace defines} $\calN$ via $\tau$ if, for each $\calN$-definable set $X$ of $\calN^n$, there is an $\calM$ definable subset $Y$ of $\calM^{kn}$ such that 
    \[(a_0,\dotsm, a_{n-1})\in X \IFF (\tau(a_0),\dotsm,\tau(a_{n-1}))\in Y.\]

    For a theory $T$, say that $T$ \textbf{trace defines} a structure $\calN$ if some model $\calM$ of $T$ trace defines $\calN$.

    $T$ \textbf{trace defines} another theory $T'$ if every model of $T'$ is trace defined by some model of $T$.
\end{definition}

We can characterize both stability and NIP by the trace definability of certain structures. Namely, 

\begin{proposition}
    \begin{enumerate}
        \item $T$ is stable if and only if $T$ does not trace define $(\bbQ,<)$.

        \item $T$ is NIP if and only if $T$ does not trace define the random graph.
    \end{enumerate}
\end{proposition}

Speaking loosely, these facts tell us that instability and IP are characterized by the occurrence of linearly ordered and random graph structures in models of their theories, respectively. It makes sense, then, that indiscernible linear orders and random graphs in these theories would not be able to forget their order or graph structure, and thus be collapsed. 

[Walsberg has some precise results on the relation between indiscernible collapse and trace definability, see section 4.2 of \cite{walsberg_notes_2021}]

However, the property of simplicity cannot be characterized by the trace definability of a structure. This is because there are instances of simple theories which are \textbf{trace maximal}, i.e., which trace define every theory. An easy example of this is the theory of generic $n$-ary relations, one for each $n$. A more natural example is the theory of pseudofinite fields. (see \cite{walsberg_notes_2021} Lemma 4.12, plus section 5.7)

Given the connection of trace definition to indiscernible collapse, this suggests that it might be impossible to characterize TP by an indiscernible collapse. Indeed, this is the case.

\begin{theorem}
    Consider any Ramsey class with a Fra\"iss\'e limit structure, $\calI$. It is not the case that a theory $T$ has the Tree Property if, and only if, in every model of $T$, all $\calI$-indexed indiscernibles are also order indiscernibles.

    \begin{proof}
    Towards a contradiction, suppose TP is, in fact, characterized by the collapse of  $\calI$-indexed indiscernibles, for some Ramsey structure $\calI$.

    Since not all theories are simple, the collapse must be non-trivial, i.e, there are quantifier-free types $q, q'$ witnessed in $\calI$ such that $q\mid_<=q'\mid_<$, yet there exist $(j_0,\dotsm, j_{n-1})=\bar{j}, (j_0',\dotsm j_{n-1}')=\bar{j}'\in \calI^n$ such that $\bar{j}\models q$, $\bar{j}\not\models q'$, $\bar{j}'\models q'$ and $\bar{j}'\not\models q$. Since $q,q'$ differ from each other, there must be a formula $\psi_q\in q$ such that $\neg\psi_q\in q'$
    
    %$\bar{j}\models \psi_q(x)\land\neg\psi_{q'}(x)$, and $\bar{j}'\models \psi_{q'}(x)\land\neg\psi_q(x)$.

    Let $T$ be a trace-maximal structure without the tree property, and let $\calM\models T$ trace define $\calI$. 

    So there is an injection $\tau\colon \calI\to \calM$ such that for each $\calI$-definable set $X$ of $\calI^n$, there is an $\calM$ definable subset $Y$ of $\calM^{kn}$ such that 
    \[(*)\enspace (a_0,\dotsm, a_{n-1})\in X \IFF (\tau(a_0),\dotsm,\tau(a_{n-1}))\in Y.\]

    Consider the image $\tau(\calI)$ as an $\calI$-indexed set $A=\{a_i\colon i\in \calI\}$ by setting $\tau(i)=a_i$. Since $\calI$ is Ramsey, $\calI$-indexed indiscernibles have the modeling property, so we may find $\calI$-indexed indiscernibles $B=\{b_i\colon i\in \calI\}$ locally based on $A$.

    We claim $B$ are not order indiscernibles, and thus contradict our assumption that all $\calI$-indexed indiscernibles collapse in models of simple theories.

    The formula $\psi_q$ defines a set $X_q$ in $\calI^n$. Since $\calM$ trace defines $\calI$, there is a definable set $Y_q$ in $\calM^{kn}$ making the schema (*) true. In particular, $Y\subseteq A^n$. Say that $Y_q$ is defined by $\vphi_q$.


    Denote by $b_{\bar{j}}$ the tuples $(b_{j_0},\dotsm ,b_{j_{n-1}})$, and likewise for other tuples. By local basedness, there are tuples $\bar{i}\bar{i}'\equiv_{qftp}\bar{j}\bar{j}'$ from $\calI$ such that $$\tp_{\vphi_q}(b_{\bar{j}}b_{\bar{j}'})=\tp_{\vphi_q}(a_{\bar{i}}a_{\bar{i}'}).$$ 

    Then, observe that we have, on the one hand, $$\bar{i}\models q\implies \models \psi_q(\bar{i}) \implies \bar{i}\in X_q\implies \tau(\bar{i})=a_{\bar{i}}\in Y_q\implies \models \vphi_q(a_{\bar{i}})\implies \models \vphi_q(b_{\bar{j}}),$$
    and on the other, 
    $$\bar{i}'\models q'\implies \models\neg\psi_q(\bar{i}') \implies \bar{i}'\notin X_q\implies \tau(\bar{i}')=a_{\bar{i}'}\notin Y_q\implies \models \neg\vphi_q(a_{\bar{i}'})\implies \models \neg\vphi_q(b_{\bar{j}'}).$$

    Thus, $\tp(b_{\bar{j}})\neq \tp(b_{\bar{j}'})$, even though the order types of $\bar{j}$ and $\bar{j}'$ are equal. Hence the indiscernible structure $B$ are not order indiscernibles, contradicting our assumption that all $\calI$-indexed indiscernibles collapse in models of simple theories.

    %Note that $\bar{i}\models q$ and $\bar{i}'\models q'$. 

    
    \end{proof}
\end{theorem}

[In fact, this theorem is a trivial corollary of the existence of trace maximal simple theories, together with the following result of Walsberg (one direction of which is essentially the proof presented here):]

\begin{proposition} (Proposition 4.15 in Walsberg's monograph)

Suppose that $\calI$ is a finely homogeneous Ramsey structure. Then $\calM$ trace defines $\calI$ via an injection $\calI\to M^m$ if, and only if, there is a small set of parameters $A$ and a non-collapsed $A$-indiscernible picture $\calI\to \calM^m$ of $\calI$ in $\calM$.
    
\end{proposition}


___________

Below: Deleted version of the main proof, materially the same:

\begin{theorem}\label{SOPn pattern theorem}
    For $n\geq 3$, a theory $T$ has $\SOP_n$ if, and only if, $T$ has $\Sigma_n$-SOP.
    
\end{theorem}

\begin{proof}
    First, suppose $T$ has $\Sigma_n$-SOP, witnessed by the formula $\psi(x,y)$ and the parameters $(a_{i,j})_{i<n, j<\omega}$. %We claim that the following formula $\vphi(\bar{y}_0, \bar{y}_1)$ witnesses $\SOP_n$, where $\bar{y}_i=(y_{i,0}, y_{i,1},\dotsm, y_{i,n-1})$:
   % \[\vphi(\bar{y}_0, \bar{y}_1)=\bigwedge_{\ell<m<n}\forall x(\psi(x, y_{0,\ell})\to \psi(x, y_{1,m}).\]
    We claim that there is a formula that witnesses $\SOP_n$ for the parameters $(\bar{a}_i)_{i<\omega}$, where $\bar{a}_i=(a_{0,i}, a_{1,i},\dotsm, a_{n-1,i})$; i.e., the parameters in the poset's ``columns," in ascending order. 
    
    %First, observe that if $i<j$, then $\vphi(\bar{a}_i, \bar{a}_j)=\bigwedge_{\ell<m<n}\forall x(\psi(x, a_{i,\ell})\to \psi(x, a_{j,m})$. So each conjunct is of the form $\forall x(\psi(x, a_{i,\ell})\to \psi(x, a_{j,m})$, where $i<j$ and $\ell<m$. In the poset $\Sigma_n$, we have $a_{i,\ell}<a_{m, j}$ whenever $\ell<m$ and $i<j$, so by $\Sigma_n$-SOP, $\models\forall x(\psi(x, a_{i,\ell})\to \psi(x, a_{j,m}))$. But observe that each conjunct of $\vphi(\bar{a}_i, \bar{a}_j)$ is of this form. Hence we have $\models \vphi(\bar{a}_i, \bar{a}_j)$. %Likewise, since $a_{j,\ell}\not<a_{i,m}$, when $i<j$ and $\ell<m$, we have $\not\models \vphi(\bar{a}_j, \bar{a}_i)$

    The witnessing formula will be an element of the $\psi$-type of the first two columns, $p(\bar{y}_0, \bar{y}_1):=\tp_\psi(\bar{a}_0, \bar{a}_1)$.

    By $\Sigma_n$-SOP, $p$ contains all formulae of the forms $\forall x(\psi(x, y_{\ell,0})\to \psi(x, y_{m,1}))$ and $\neg \forall x(\psi(x, y_{m,0})\to \psi(x, y_{\ell, 1}))$, for all $\ell<m<n$. Thus, since these same relations hold between arbitrary columns of the $\Sigma_n$-SOP witness, we have $(\bar{a}_i,\bar{a}_j)\models p(\bar{y}_0,\bar{y}_1)$ if and only if $i<j$.

    To check that we can have no loops of length less than $n+1$ in any formula in $p$, consider the type %the $\psi$-type of the first two columns, $p(\bar{y}_0, \bar{y}_1)=\tp_\psi(\bar{a}_0, \bar{a}_1)$. If \[\{\vphi(\bar{y}_0,\bar{y}_1), \vphi(\bar{y}_1,\bar{y}_2),\dotsm, \vphi(\bar{y}_{n-2},\bar{y}_{n-1}), \vphi(\bar{y}_{n-1},\bar{y}_0)\}\] is consistent, it follows that 
    \[Q(\bar{y}_0,\dotsm, \bar{y}_{n-1})=p(\bar{y}_0,\bar{y}_1)\cup p(\bar{y}_1,\bar{y}_2)\cup\dotsm \cup p(\bar{y}_{n-2},\bar{y}_{n-1})\cup p(\bar{y}_{n-1},\bar{y}_0.)\] %is consistent, since $\vphi$ implies all of the $\psi$-relations between $\bar{a}_0$ and $\bar{a}_1$.

    Now, $Q$ includes the following chain of implications:

    \[\forall x(\psi(x, y_{0,1})\to \psi(x, y_{1,2})), \forall x(\psi(x, y_{1,2})\to \psi(x, y_{2,3})), \dotsm \forall x(\psi(x, y_{n-2,n-1})\to \psi(x, y_{n-1,0})).\]

    [Include diagram??]

    Thus, this type implies $\forall x(\psi(x, y_{0,1})\to \psi(x, y_{n-1,0}))$. But since $(n-1,0)\not<(0,1)$ in $\Sigma_n$, we also have that $\neg \forall x(\psi(x, y_{n-1,0})\to \psi(x, y_{0, 1}))\in p(\bar{y}_0,\bar{y}_1)\subseteq Q(\bar{y}_0,\dotsm, \bar{y}_{n-1})$. Hence $Q$ is inconsistent. By compactness, we may conclude that $Q$ is finitely inconsistent, thus there is a formula $\vphi(\bar{y}_0,\bar{y}_1)\in p$ which witnesses $\SOP_n$ for this sequence of parameters.
    
%    By $\Sigma_n$-SOP, this formula can only be in $\tp_\psi(\bar{a}_0, \bar{a}_1)$ if $(1,0)<a_{0, n-1}$ in $\Sigma_n$; since this relation does not hold, we have a contradiction. Thus, $\vphi(\bar{y}_0, \bar{y}_1)$ witnesses $\SOP_n$.




    Conversely, suppose that $\vphi(x,y)$ witnesses $\SOP_n$. By compactness, we may assume it witnesses $\SOP_n$ on parameters indexed by $(\bbQ,<)$, say $(a_q)_{q\in\bbQ}$ in $\bbM\models T$; take these parameters to have length $k$. %The formula witnessing $\Sigma_n$-SOP will be a disjunction built from $n-1$-many formulas, each of which, along with the parameters witnessing $\SOP_n$ defines the nodes at a particular level of the poset.
   %[ For all of the levels $k$ other than the lowest (0th) one, we want the sets defined at level $k$ to consist of those elements which can be [necessary??]]   
   % For $0<k<n$, define the following formula expressing that there is a length at most $k$ path of $\vphi$-relations from $x$ to $z$: 
  %  \[\vphi_k(x,z)=\vphi(x,z)\lor\bigvee_{i=0}^{k-2}\exists y_0\dotsm \exists y_i\left[\vphi(x,y_0)\land \vphi(y_i,z)\land \bigwedge_{j=0}^i\vphi(y_j,y_{j+1})\right].\]
As Garcia and Mennuni note (their Proposition 1.4), $T$ has $\Sigma$-SOP if, and only if, $\bbM\models T$ interprets a poset $\Sigma'$ into which $\Sigma$ embeds. We show that $\bbM$ interprets a poset into which $\Sigma_n$ embeds. 

Fixing distinct arbitrary parameters $c_0,\dots, c_{n-1}$ from $\bbM$, the domain for the poset consists of $n$ levels, given by the $c_i$. The domain set is $P=\bigcup_{i<n}\{c_i\}\times\bbM^k$. The poset relation is defined between pairs of variables $(z,\bar{x})$, where $\bar{x}$ has length $k$ and $z$ has length 1. It expresses the relation that holds between $(c_i, \bar{b}_0)$ and $(c_{i'},\bar{b}_1)$ when $i<i'$ and there is a $i'-i$-length path in the $\vphi$-relation starting with $\bar{b}_0$ and ending with $\bar{b}_1$.

    \[\psi(z,\bar{x};w,\bar{y})=(\bar{x}=\bar{y}\land z=w)\lor\]

    \[\bigvee_{i<i'<n}\left((z=c_i
    \land w=c_i')\land \exists \bar{u}_0,\dotsm, \bar{u}_{i'-i-1}\left[\bar{x}=\bar{u}_0\land \bar{y}=\bar{u}_{i'-i-1}\land \bigwedge_{\ell<i'-i-1}\vphi(\bar{u}_\ell, \bar{u}_{\ell+1})\right]\right).\]

    This formula defines a poset relation $\preceq$ on $P$ by definition, so it suffices to show that $\Sigma_n$ embeds into $(P,\preceq)$. We claim that the function $h\colon \Sigma_n\to (P,\prec)$ defined by $h((i,j))=(c_i, a_j)$ gives the desired embedding.

    To check that $h$ is an embedding, first suppose $(i,j)\leq(i',j')$. If $(i,j)=(i',j)$, then $h((i,j))\preceq h((i',j'))$, by the first disjunct of $\psi$. So we may assume $(i,j)<(i',j)$; hence $i<i' <n-1$ and $j<j'$. Since $\bbQ$ is dense, we may find $q_0<q_1<\dotsm <q_{i-i'-1}$ with $j=q_0$ and $j'=q_{i-i'-1}$. We have $\vphi(a_{q_0}, a_{q_1}), \vphi(a_{q_1},a_{q_2}),\dotsm, \vphi(a_{q_{i-i'-2}},a_{q_{i-i'-1}})$, and thus $\models \psi(c_i,a_j;c_{i'},a_{j'})$. Thus we have that $h((i,j))\prec h((i',j'))$; so in either case, $h((i,j))\preceq h((i',j'))$
    
    Now, suppose that $(i,j)\not\leq(i'j')$. Then at least one of $i\geq i'$ and $j\geq j'$ is true. If $i>i'$, then there is no disjunct of $\psi$ that could make $\psi(c_i,a_j;c_{i'},a_{j'})$ true, by the equality conditions on the $c_k$ parameters. If $i=i'$ we must look to the first conjunct of $\psi$, and since in this case $j\neq j'$, we have $\not\models \psi(c_i,a_j;c_{i'},a_{j'})$. Finally, suppose $i<i'$ and $j\geq j'$. If we had $\models \psi(c_i,a_j;c_{i'},a_{j'})$, then it would follow that there is a $i'-i$-length $\vphi$-path from $a_{j'}$ to $a_j$. The fact that $\vphi$ witnesses $\SOP_n$ on $(a_q)_{q\in\bbQ}$ implies that we also have $\models \vphi(a_j,a_{j'})$. But together with the links in the $i'-i<n$-length $\vphi$ path, this would show that there is a length $\leq n$ $\vphi$-loop, contradicting $\SOP_n$'s condition that such loops are inconsistent. Thus in any case we must have $h((i,j))\not\preceq h((i'j'))$. We conclude that $h$ is an embedding of posets, and thus that $T$ has $\Sigma_n$-SOP.
    
\end{proof}

We have now proved that the $\SOP_n$ properties are poset characterizable. It immediately follows by Proposition \ref{poset implies straight} that the $\SOP_n$s are straightly definable. [mention here or elsewhere Shelah's mistaken claim to have proven this, and the fact that it has already been shown for $\SOP_3$, see references on Bailetti p3]

\begin{theorem}
    For $n\geq 3$, $\SOP_n$ is straightly definable.
\end{theorem}

\begin{proof}
    By Theorem \ref{SOPn pattern theorem}, each $\SOP_n$ is poset-characterizable. Thus by Proposition \ref{poset implies straight}, $\SOP_n$ is straightly definable.
\end{proof}

==> unused_diagrams.tex <==
\begin{center}
\begin{tikzpicture}
    \node(b0){$b_0$};
    \node(b1)[right of = b0]{$b_1$};
    \node(dots1)[right of =b1]{$b_2$};
    \node(bi)[right of = dots1]{$b_3$};
    \node(bi+1)[right of=bi]{$b_{4}$};
    \node (dots2)[right of =bi+1]{...};
    \node(satisfied)[above of = dots1]{$M\models \vphi(b_0,b_{4})$};
    \node(unsatisfied)[below of = dots1]{$M\not\models\vphi (b_{4},b_0)$};
    \draw[thick] (satisfied) -- (b0);
    \draw[thick, ->] (satisfied) -- (bi+1);
    \draw[dashed, ->] (unsatisfied) -- (b0);
    \draw[dashed] (unsatisfied) -- (bi+1);    
\end{tikzpicture}
\end{center}




%\[
%\begin{array}{c|ccccc}
 % \varphi(a_i,\,b_j) & b_0 & b_1 & b_2 & b_3 & b_4 \\[2pt]
 % \hline\rule{0pt}{2.4ex}
 % a_0 & \circ & \bullet & \bullet & \bullet & \bullet \\
%  a_1 & \circ & \circ   & \bullet & \bullet & \bullet \\
 % a_2 & \circ & \circ   & \circ   & \bullet & \bullet \\
%  a_3 & \circ & \circ   & \circ   & \circ   & \bullet \\
 % a_4 & \circ & \circ   & \circ   & \circ   & \circ   \\[2pt]
%\end{array}
%\]
% \bullet = holds, \circ = fails


%Below, we visualize part of the order property, as defined in terms of the tuples $(a_i, b_i)_{i< \omega}$; here $\bullet$ denotes $M \models \varphi(a_{i}, b_{j})$ and $\circ$ denotes $M \models \neg\varphi(a_{i}, b_{j})$.%\footnote{ Generative AI was used in constructing some of the diagrams in this paper.}--think we just need to acknowledge this for the journal submission%


\begin{center}
\begin{tikzpicture}[scale=1.3]
  \draw[draw=black, line width=0.4pt]
    (0,0) ellipse (3.95cm and 1.90cm);
  \draw[draw=black, line width=0.4pt]
    (0,0) ellipse (2.75cm and 1.32cm);
  \draw[draw=black, line width=0.4pt]
    (0,0) ellipse (1.70cm and 0.80cm);
  \draw[draw=black, line width=0.4pt]
    (0,0) ellipse (0.65cm and 0.38cm);
  \node[font=\small] at ( -.15, 0.00) {$\varphi(M,a_0)$};
  \node[font=\small] at (-1.22, 0.00) {$\varphi(M,a_1)$};
  \node[font=\small] at (-2.25, 0.00) {$\varphi(M,a_2)$};
  \node[font=\small] at (-3.42, 0.00) {$\varphi(M,a_3)$};
\end{tikzpicture}
\end{center}


\begin{figure}[!ht]
\centering
\resizebox{1\textwidth}{!}{%
\begin{circuitikz}
\tikzstyle{every node}=[font=\fontsize{18.2pt}{23.7pt}\selectfont]
\draw  (3,5.5) circle (0.125cm);
\draw  (4,5.5) circle (0.125cm);
\draw  (5,5.5) circle (0.125cm);
\draw  (3,4.5) circle (0.125cm);
\draw  (4,4.5) circle (0.125cm);
\draw  (5,4.5) circle (0.125cm);
\draw  (3,3.5) circle (0.125cm);
\draw  (4,3.5) circle (0.125cm);
\draw  (5,3.5) circle (0.125cm);
\draw  (3,2.5) circle (0.125cm);
\draw  (4,2.5) circle (0.125cm);
\draw  (5,2.5) circle (0.125cm);
\node [font=\fontsize{9.1pt}{11.8pt}\selectfont, inner xsep=0.080cm, inner ysep=0.085cm, rounded corners=0.000cm] at (6.375,4.125) {$\cdot\cdot\cdot$};
\draw  (7.875,5.5) circle (0.125cm);
\draw  (7.875,4.5) circle (0.125cm);
\draw  (7.875,3.5) circle (0.125cm);
\draw  (7.875,2.5) circle (0.125cm);
\node [font=\fontsize{9.1pt}{11.8pt}\selectfont, inner xsep=0.080cm, inner ysep=0.085cm, rounded corners=0.000cm] at (10,4.125) {$\cdot\cdot\cdot$};
\draw [-{Stealth[scale=1.5]}, ] (3.0884,5.4116) -- (3.9116,4.5884);
\draw [-{Stealth[scale=1.5]}, ] (3.125,5.5) -- (4.9116,4.5884);
\draw [-{Stealth[scale=1.5]}, ] (3.0884,4.4116) -- (4,3.625);
\draw [-{Stealth[scale=1.5]}, ] (3.125,4.5) -- (4.9116,3.5884);
\draw [-{Stealth[scale=1.5]}, ] (3.0884,3.4116) -- (3.9116,2.5884);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,3.4116) -- (4.9116,2.5884);
\draw [-{Stealth[scale=1.5]}, ] (3.125,3.5) -- (4.9116,2.5884);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,4.4116) -- (4.9116,3.5884);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,5.4116) -- (4.9116,4.5884);
\draw [-{Stealth[scale=1.5]}, ] (3.0884,3.4116) -- (7.75,2.5);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,3.4116) -- (7.75,2.5);
\draw [-{Stealth[scale=1.5]}, ] (5.0884,3.4116) -- (7.75,2.5);
\draw [-{Stealth[scale=1.5]}, ] (3.0884,4.4116) -- (7.75,3.5);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,4.4116) -- (7.75,3.5);
\draw [-{Stealth[scale=1.5]}, ] (5.0884,4.4116) -- (7.75,3.5);
\draw [-{Stealth[scale=1.5]}, ] (3.0884,5.4116) -- (7.75,4.5);
\draw [-{Stealth[scale=1.5]}, ] (4.0884,5.4116) -- (7.75,4.5);
\draw [-{Stealth[scale=1.5]}, ] (5.0884,5.4116) -- (7.75,4.5);
\end{circuitikz}
}%
\label{fig:my_label}
\end{figure}
    

